Non-prehensile Planar Manipulation via Trajectory Optimization with Complementarity Constraints

Contact adaption is an essential capability when manipulating objects. Two key contact modes of non-prehensile manipulation are sticking and sliding. This paper presents a Trajectory Optimization (TO) method formulated as a Mathematical Program with Complementarity Constraints (MPCC), which is able to switch between these two modes. We show that this formulation can be applicable to both planning and Model Predictive Control (MPC) for planar manipulation tasks. We numerically compare: (i) our planner against a mixed integer alternative, showing that the MPCC planer converges faster, scales better with respect to time horizon, and can handle environments with obstacles; (ii) our controller against a state-of-the-art mixed integer approach, showing that the MPCC controller achieves better tracking and more consistent computation times. Additionally, we experimentally validate both our planner and controller with the KUKA LWR robot on a range of planar manipulation tasks.

==> Makefile <==
# Makefile for compiling a *.tex file into a *.pdf file
# The current folder must contain only one *.tex file
#
# Author: Joao Moura
# Email: jpousad@ed.ac.uk
# Last Modified at 31/03/2021
#
#################################################################
#################################################################
# Identify what is the name of the *.tex file to compile
# NOTE: There must be a single *.tex file in the current directory
TEX = pdflatex --shell-escape
BIB = biber
TIKZ = Tikz
FILE_TEX=$(wildcard *.tex)
FILE_BIB=bib.bib
TARGET=$(FILE_TEX:.tex=)
#################################################################

#################################################################
# Rule that runs whether the make is called or the target file is outdated.
# FORCE: $(FILE_TEX) $(TARGET).bbl
FORCE: $(FILE_TEX)
	$(TEX) $(TARGET)

# $(TARGET).bbl: $(FILE_TEX) $(FILE_BIB)
	# $(BIB) $(TARGET)
#################################################################

#################################################################
# Rule to create a bibtex file
.PHONY: bib
bib:
	$(BIB) $(TARGET)
#################################################################

#################################################################
# Rule for cleaning: It removes all the files with TARGET name except the file with *.tex extension
.PHONY: clean
clean: 
	rm -f $(filter-out $(TARGET).tex, $(wildcard $(TARGET).*))
#################################################################

#################################################################
# Rule for cleaning all tikz files
.PHONY: cleanall
cleanall: 
	rm -f $(filter-out $(wildcard Tikz/*.tex) $(TARGET).tex, $(wildcard Tikz/*.*) $(wildcard $(TARGET).*))
#################################################################

#################################################################
# Rule for cleaning the bib file
.PHONY: cleanbib
cleanbib:
	# Remove unnecessary keywords:
	gsed -i '/^month/d' $(FILE_BIB)
	gsed -i '/^abstract/d' $(FILE_BIB)
	gsed -i '/^archivePrefix/d' $(FILE_BIB)
	gsed -i '/^arxivId/d' $(FILE_BIB)
	gsed -i '/^eprint/d' $(FILE_BIB)
	gsed -i '/^isbn/d' $(FILE_BIB)
	gsed -i '/^issn/d' $(FILE_BIB)
	gsed -i '/^mendeley-tags/d' $(FILE_BIB)
	gsed -i '/^pmid/d' $(FILE_BIB)
	gsed -i '/^primaryClass/d' $(FILE_BIB)
	gsed -i '/^keywords/d' $(FILE_BIB)
	gsed -i '/^url/d' $(FILE_BIB)
	gsed -i '/^file/d' $(FILE_BIB)
	# Insert tab before keyword:
	gsed -i 's/^\([a-z]\)/\t\1/' $(FILE_BIB)
	# Remove double brackets in titles:
	gsed -i 's/{{\(.*\)}}/{\1}/' $(FILE_BIB)
	# Add a line after each reference:
	gsed -i '/^}/a\\' $(FILE_BIB)
#################################################################


==> Tikz/tikz.tex <==
% function to compute angle and length between coordinates
\makeatletter
\newcommand{\getLengthAndAngle}[2]{%
    \pgfmathanglebetweenpoints{\pgfpointanchor{#1}{center}}
                              {\pgfpointanchor{#2}{center}}
    \global\let\myangle\pgfmathresult % we need a global macro
    \pgfpointdiff{\pgfpointanchor{#1}{center}}
                 {\pgfpointanchor{#2}{center}}
    \pgf@xa=\pgf@x % no need to use a new dimen
    \pgf@ya=\pgf@y
    \pgfmathparse{veclen(\pgf@xa,\pgf@ya)/28.45274} % to convert from pt to cm
    \global\let\mylength\pgfmathresult % we need a global macro
}
\makeatother 
\tikzset{%
    pics/pivot/.style args={#1,#2}{%
        code = {%
            % #1: radius of small circle (pin);
            % #2: radius of large circle (outer dimension).
            %\draw[thick, fill=white] (-#2,#2) -- (-#2,0) arc(180:360:#2) -- (#2,#2) -- cycle;
            \draw[thick, fill=white] (#2,-#2) -- (#2,0) arc(0:180:#2) -- (-#2,-#2) -- cycle;
            \draw[thick, fill=gray] (0,0) circle circle (#1);
        }
    },
    ground/.style = {fill,pattern=north east lines,draw=none,minimum width=1cm,minimum height=1cm},
    spring/.style = {thick,decorate,decoration={zigzag,pre length=0.3cm,post length=0.3cm,segment length=6}},
    damper/.style = {thick, decoration={markings, mark connection node=dmp, mark=at position 0.5 with
              {%
                \node (dmp) [thick,inner sep=0pt,transform shape,rotate=-90,minimum width=15pt,minimum height=3pt,draw=none] {};
                \draw [thick] ($(dmp.north east)+(2pt,0)$) -- (dmp.south east) -- (dmp.south west) -- ($(dmp.north west)+(2pt,0)$);
                \draw [thick] ($(dmp.north)+(0,-5pt)$) -- ($(dmp.north)+(0,5pt)$);
              }
        }, decorate},
%    \tikzstyle{damper}=[thick, decoration={markings, mark connection node=dmp, mark=at position 0.5 with
%       {
%         \node (dmp) [thick,inner sep=0pt,transform shape,rotate=-90,minimum width=15pt,minimum height=3pt,draw=none] {};
%         \draw [thick] ($(dmp.north east)+(2pt,0)$) -- (dmp.south east) -- (dmp.south west) -- ($(dmp.north west)+(2pt,0)$);
%         \draw [thick] ($(dmp.north)+(0,-5pt)$) -- ($(dmp.north)+(0,5pt)$);
%       }
%     }, decorate]
    pics/dimLinear/.style args={#1,#2,#3,#4,#5,#6,#7}{%
        code = {%
            % #1: node 1
            % #2: node 2
            % #3: node 1 guide line distance
            % #4: node 2 guide line distance
            % #5: label distance
            % #6: label
            % #7: label position (ex: right, left, above, below)
            \draw[very thin, gray] ($(#1)!#3!-90:(#2)$) -- ($(#1)!#5+3pt!-90:(#2)$); % lateral line perpendicular to nodes 1 and 2
            \draw[very thin, gray] ($(#2)!#4!90:(#1)$) -- ($(#2)!#5+3pt!90:(#1)$); % lateral line perpendicular to nodes 1 and 2
            \draw[very thin, arrows=<->, gray] ($(#1)!#5!-90:(#2)$) -- ($(#2)!#5!90:(#1)$) node[midway, #7] {#6}; % dimension line parallel to nodes 1 and 2
        }
    },
    pics/dimAngular/.style args={#1,#2,#3,#4,#5,#6,#7,#8}{%
        code = {%
            % #1: node 1 (this node will define the distance the arc from the central node)
            % #2: node 2
            % #3: node centre
            % #4: distance before arrow ends
            % #5: node 1 guide line distance
            % #6: label
            % #7: label position (ex: right, left, above, below)
            % Create lines for computing arc centre
            \def\argone{#4}\def\argtwo{0}
            \ifx\argone\argtwo % if the arrow offset is zero the rotation centre remains the same
                \coordinate (centre) at (#3);
            \else % if there is offset we find the:
                \draw[name path=AB,draw=none] ($(#2)!#4!90:(#3)$) -- ($(#3)!#4!-90:(#2)$); % line parallel to the link formed by the nodes 1 and 2 with offset #4
                \draw[name path=CD,draw=none] (#1) -- (#3); % reference line for measure the angle
                \coordinate [name intersections={of={AB and CD}}]; % intersection between the offset line and the reference line
                \coordinate (centre) at (intersection-1); % set the rotation centre as the found intersection
            \fi
            \draw [very thin, gray, #8] let
                \p0 = ($(#1)-(centre)$), % difference vector between reference and centre
                \p1 = ($($(#2)!#4!90:(#3)$)-(centre)$) % difference vector reference between the offset line and the centre
                in (#1) arc [start angle={atan2(\y0,\x0)}, end angle={atan2(\y1,\x1)}, radius=({veclen(\y0,\x0)})] node[midway, #7] {#6}; % angular dimension line
            \draw[very thin, gray] ($(#3)!#5!0:(#1)$) -- ($(#1)!-3pt!0:(#3)$); % Draw guide line
        }
    },
    pics/link/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: node 1
            % #2: node 2
            % #3: characteristic dimension of drawing
            % #4: opacity of the link
            \draw[thick, fill=white, opacity=#4] ($(#1)!1.5*#3!-90:(#2)$) -- ($(#2)!1.5*#3!90:(#1)$) -- ($(#2)!1.5*#3!-90:(#1)$) -- ($(#1)!1.5*#3!90:(#2)$) -- cycle; % lines parallel to nodes 1 and 2
            \fill[white, draw=none] (#2) circle circle (2.5*#3); % outer round part
            \draw[thick, opacity=#4] (#2) circle circle (2.5*#3); % outer round part
            \fill[gray, draw=none, fill opacity=#4] (#2) circle circle (#3);
            \draw[thick, opacity=#4] (#2) circle circle (#3);
        }
    },
    pics/linkwithbreak/.style args={#1,#2,#3,#4,#5}{%
        code = {%
            % #1: node 1
            % #2: node 2
            % #3: characteristic dimension of drawing
            % #4: opacity of the link
            \draw[thick, fill=white, opacity=#4] ($(#1)!1.5*#3!-90:(#2)$) -- ($(#2)!1.5*#3!90:(#1)$) -- ($(#2)!1.5*#3!-90:(#1)$) -- ($(#1)!1.5*#3!90:(#2)$); % lines parallel to nodes 1 and 2
            \draw[very thin,line cap=round] ($(#1)!1.5*#3!-90:(#2)$) to [out=45+#5,in=-135+#5, thin] ($(#1)!1.5*#3!90:(#2)$);
            \fill[white, draw=none] (#2) circle circle (2.5*#3); % outer round part
            \draw[thick, opacity=#4] (#2) circle circle (2.5*#3); % outer round part
            \fill[gray, draw=none, fill opacity=#4] (#2) circle circle (#3);
            \draw[thick, opacity=#4] (#2) circle circle (#3);
        }
    },
    pics/centreofmass/.style args={#1,#2}{%
        code = {%
            % #1: radius of symbol
            \draw[fill=black, thin] (#2) -- ++(#1,0) arc [radius=#1, start angle=0,end angle=90] -- ++(0,-2*#1) arc [radius=#1, start angle=270, end angle=180] -- cycle;
            \draw[thin] (#2) circle circle (#1);
        }
    },
    pics/lastlink/.style args={#1,#2,#3}{%
        code = {%
            % #1: node 1
            % #2: node 2
            % #3: characteristic dimension of drawing
            \draw[thick] ($(#1)!1.5*#3!-90:(#2)$) -- ($(#2)!1.5*#3!90:(#1)$);
            \draw[thick] ($(#1)!1.5*#3!90:(#2)$) -- ($(#2)!1.5*#3!-90:(#1)$);
            % End-effentor
            \draw[ultra thick,rounded corners=#3] ($($(#2)!2*#3!180:(#1)$)!3*#3!-90:(#1)$) -- ($(#2)!3*#3!-90:(#1)$) -- (#2) -- ($(#2)!3*#3!90:(#1)$) -- ($($(#2)!2*#3!180:(#1)$)!3*#3!90:(#1)$);
        }
    },
    pics/foot/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: node 1
            % #2: node 2
            % #3: characteristic dimension of drawing
            % #4: opacity of the link
            \draw[fill=white, very thick, rounded corners=#3, opacity=#4] ($(#1)!5.0*#3!-90:(#2)$) -- ($(#2)!1.5*#3!90:(#1)$) -- ($(#2)!1.5*#3!-90:(#1)$) -- ($(#1)!5.0*#3!90:(#2)$) -- cycle;
            % End-effentor
            \fill[white, draw=none] (#2) circle circle (2.5*#3); % outer round part
            \draw[thick, opacity=#4] (#2) circle circle (2.5*#3); % outer round part
            \fill[gray, draw=none, fill opacity=#4] (#2) circle circle (#3);
            \draw[thick, opacity=#4] (#2) circle circle (#3);
        }
    },
    pics/lastlinklinecontact/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: node 1
            % #2: node 2
            % #3: characteristic dimension of drawing
            % #4: opacity of the link
            % ------------------------------
            % computing angle between nodes
            \pgfmathanglebetweenpoints{\pgfpointanchor{#1}{center}}{\pgfpointanchor{#2}{center}}
            \edef\angle{\pgfmathresult}
            % coordinates
            \coordinate (bottomRight) at ($(#2)!1.5*#3!90:(#1)$);
            \coordinate (bottomLeft) at ($(#1)!1.5*#3!-90:(#2)$);
            \coordinate (topRight) at ($(#2)!1.5*#3!-90:(#1)$);
            \coordinate (topLeft) at ($(#1)!1.5*#3!90:(#2)$);
            \coordinate (bottomMiddle) at ($(bottomRight)!2.0*#3!0:(bottomLeft)$);
            \coordinate (topMiddle) at ($(topRight)!2.0*#3!0:(topLeft)$);
            \coordinate (bottomBase) at ($(bottomRight)!2.0*#3!180:(topRight)$);
            \coordinate (topBase) at ($(topRight)!2.0*#3!180:(bottomRight)$);
            % drawing
            % \draw[thick, opacity=#4] (bottomLeft) -- (bottomMiddle);
            % \draw[thick, opacity=#4] (topLeft) -- (topMiddle);
            \draw[thick, opacity=#4, fill=white] (bottomLeft) -- (bottomMiddle) -- (topMiddle) -- (topLeft);
            % \draw[thick, opacity=#4] (topLeft) -- (topMiddle);
            % End-effentor
            \draw[thick, fill=gray, opacity=#4, fill opacity=#4, rounded corners=0.5pt] (bottomMiddle)  to [out=\angle-90,in=\angle+135] (bottomBase) -- (topBase) to [out=\angle-135,in=\angle+90] (topMiddle) -- cycle;
        }
    },
    pics/lastlinkpointcontact/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: node 1
            % #2: node 2
            % #3: characteristic dimension of drawing
            % coordinates
            \coordinate (bottomLeft) at ($(#1)!1.5*#3!-90:(#2)$);
            \coordinate (bottomRight) at ($(#2)!1.5*#3!90:(#1)$);
            \coordinate (topLeft) at ($(#1)!1.5*#3!90:(#2)$);
            \coordinate (topRight) at ($(#2)!1.5*#3!-90:(#1)$);
            \coordinate (bottomRight2) at ($(bottomRight)!5.0*#3!0:(bottomLeft)$);
            \coordinate (topRight2) at ($(topRight)!5.0*#3!0:(topLeft)$);
            \coordinate (bottomRight3) at ($(bottomRight)!2.5*#3!0:(bottomLeft)$);
            \coordinate (topRight3) at ($(topRight)!2.5*#3!0:(topLeft)$);
            \pgfmathanglebetweenpoints{\pgfpointanchor{#1}{center}}{\pgfpointanchor{#2}{center}}
            \edef\angle{\pgfmathresult}
            % drawing
            \draw[thick, opacity=#4] (bottomLeft) -- (bottomRight2);
            \draw[thick, opacity=#4] (topLeft) -- (topRight2);
            % End-effentor
            \draw[thick, fill=gray, opacity=#4, fill opacity=#4] (topRight2) arc (\angle+90:\angle-90:1.5*#3) {[rounded corners=1.5pt] -- (bottomRight3)} arc (\angle+180:\angle+90:1.5*#3) coordinate (prov) {[rounded corners=1.5pt] arc (\angle+270:\angle+180:1.5*#3)} -- cycle;
            \draw[thick, opacity=#4] (prov) -- (#2);
            \fill[black, fill opacity=#4] (#2) circle (0.5pt);
        }
    },
    pics/limb/.style args={#1,#2,#3,#4,#5}{%
        code = {%
            % #1: point coordinate 1
            % #2: point coordinate 2
            % #3: thickness of ellipse: 0 - line; 1 - circle
            % #4: scale: 1 is no scale
            % #5: opacity of line
            % compute myangle and mylength:
            \getLengthAndAngle{#1}{#2}
            % compute central coordinate:
            \coordinate (centre) at ($(#1)!0.5!(#2)$);
            % draw limb
            \draw[rotate=\myangle,shift={(centre)}, very thick, fill=white, opacity=#5, fill opacity=1.0] (0,0) ellipse ({#4*0.5*\mylength} and {#4*#3*0.5*\mylength});
        }
    },
    pics/rect/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: square centre coordinate
            % #2: inclination angle
            % #3: rectangle x size length
            % #4: rectangle y size length
            % ------------------------------
            % draw limb
            \draw[cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}, thick, rounded corners=0.5pt] ($(#1)+(axis direction cs:0.5*#3,0.5*#4)$) rectangle ($(#1)+(axis direction cs:-0.5*#3,-0.5*#4)$);
            \draw[->, black, thick, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] (#1) --++ (axis direction cs:0.45*#3,0);
            \fill[black] (#1) circle[radius=1.5pt];
        }
    },
    pics/rectObj/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: square centre coordinate
            % #2: inclination angle
            % #3: rectangle x size length
            % #4: rectangle y size length
            % ------------------------------
            % draw limb
            \shadedraw[shading angle=#2, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}, thick, rounded corners=0.5pt] ($(#1)+(axis direction cs:0.5*#3,0.5*#4)$) rectangle ($(#1)+(axis direction cs:-0.5*#3,-0.5*#4)$);
            \draw[->, black, thick, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] (#1) --++ (axis direction cs:0.45*#3,0);
            \fill[black] (#1) circle[radius=1.5pt];
        }
    },
    pics/rectGoal/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: square centre coordinate
            % #2: inclination angle
            % #3: rectangle x size length
            % #4: rectangle y size length
            % ------------------------------
            % draw limb
            \draw[very thick, dashed, rounded corners=0.5pt, black!20!red, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] ($(#1)+(axis direction cs:0.5*#3,0.5*#4)$) rectangle ($(#1)+(axis direction cs:-0.5*#3,-0.5*#4)$);
            \draw[->, black!20!red, thick, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] (#1) --++ (axis direction cs:0.45*#3,0);
            \fill[black] (#1) circle[radius=1.5pt];
        }
    },
    pics/rectStart/.style args={#1,#2,#3,#4}{%
        code = {%
            % #1: square centre coordinate
            % #2: inclination angle
            % #3: rectangle x size length
            % #4: rectangle y size length
            % ------------------------------
            % draw limb
            \draw[very thick, dashed, rounded corners=0.5pt, black!50!green, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] ($(#1)+(axis direction cs:0.5*#3,0.5*#4)$) rectangle ($(#1)+(axis direction cs:-0.5*#3,-0.5*#4)$);
            \draw[->, black!50!green, thick, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] (#1) --++ (axis direction cs:0.45*#3,0);
            \fill[black] (#1) circle[radius=1.5pt];
        }
    },
    pics/square/.style args={#1,#2,#3}{%
        code = {%
            % #1: square centre coordinate
            % #2: inclination angle
            % #3: square size length
            % ------------------------------
            % draw limb
            \shadedraw[shading angle=#2, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}, thick, rounded corners=0.5pt] ($(#1)+(0.5*#3,0.5*#3)$) rectangle ($(#1)+(-0.5*#3,-0.5*#3)$);
            \draw[-latex, black!50!green, thick, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] (#1) --++ (0.45*#3,0);
            \fill[black] (#1) circle (1.5pt);
        }
    },
    pics/conveyercircle/.style args={#1,#2,#3}{%
        code = {%
            % #1: conveyercircle centre coordinate
            % #2: inclination angle
            % #3: conveyercircle size length
            % ------------------------------
            % draw circle
            \draw[black,fill=black] (#1) circle (0.8*#3);
            \draw[fill=gray!10!white] (#1) circle (0.4*#3);
            \draw[fill=gray!10!white, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] ($(#1)+(0.6*#3,0)$) circle (1pt);
            \draw[fill=gray!10!white, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] ($(#1)+(0,0.6*#3)$) circle (1pt);
            \draw[fill=gray!10!white, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] ($(#1)+(-0.6*#3,0)$) circle (1pt);
            \draw[fill=gray!10!white, cm={cos(-#2) ,-sin(-#2) ,sin(-#2) ,cos(-#2) ,(#1)}] ($(#1)+(0,-0.6*#3)$) circle (1pt);
        }
    },
}


==> git-latexdiff <==
#! /bin/bash

# Main author: Matthieu Moy <git@matthieu-moy.fr>
# (See the Git history for other contributors)
#
# BSD 2-Clause License
# 
# Copyright (c) 2012 - 2020, Matthieu Moy
# All rights reserved.
# 
# Redistribution and use in source and binary forms, with or without
# modification, are permitted provided that the following conditions are met:
# 
# 1. Redistributions of source code must retain the above copyright notice, this
#    list of conditions and the following disclaimer.
# 
# 2. Redistributions in binary form must reproduce the above copyright notice,
#    this list of conditions and the following disclaimer in the documentation
#    and/or other materials provided with the distribution.
# 
# THIS SOFTWARE IS PROVIDED BY THE COPYRIGHT HOLDERS AND CONTRIBUTORS "AS IS"
# AND ANY EXPRESS OR IMPLIED WARRANTIES, INCLUDING, BUT NOT LIMITED TO, THE
# IMPLIED WARRANTIES OF MERCHANTABILITY AND FITNESS FOR A PARTICULAR PURPOSE ARE
# DISCLAIMED. IN NO EVENT SHALL THE COPYRIGHT HOLDER OR CONTRIBUTORS BE LIABLE
# FOR ANY DIRECT, INDIRECT, INCIDENTAL, SPECIAL, EXEMPLARY, OR CONSEQUENTIAL
# DAMAGES (INCLUDING, BUT NOT LIMITED TO, PROCUREMENT OF SUBSTITUTE GOODS OR
# SERVICES; LOSS OF USE, DATA, OR PROFITS; OR BUSINESS INTERRUPTION) HOWEVER
# CAUSED AND ON ANY THEORY OF LIABILITY, WHETHER IN CONTRACT, STRICT LIABILITY,
# OR TORT (INCLUDING NEGLIGENCE OR OTHERWISE) ARISING IN ANY WAY OUT OF THE USE
# OF THIS SOFTWARE, EVEN IF ADVISED OF THE POSSIBILITY OF SUCH DAMAGE.
#
# git-latexdiff is a wrapper around latexdiff
# (http://www.ctan.org/pkg/latexdiff) that allows using it to diff two
# revisions of a LaTeX file.
#
# The script internally checks out the full tree for the specified
# revisions, calls latexpand to flatten the document and then calls
# latexdiff-so (if available, otherwise latexdiff). Therefore,
# this works if the document is split into multiple .tex files.
#
# Try "git latexdiff -h" for more information.
#
# To install, just copy git-latexdiff in your $PATH.

# Missing features (patches welcome ;-):
# - diff the index
# - hardlink temporary checkouts as much as possible

# Alternatives:
#
# There is another script doing essentially the same here:
# https://github.com/cawka/latexdiff/blob/master/latexdiff-git
# My experience is that latexdiff-git is more buggy than
# git-latexdiff, but they probably just don't have the same bugs ;-)
#
# There are a bunch of other alternatives cited here:
#
#   http://tex.stackexchange.com/questions/1325/using-latexdiff-with-git
#
# Ideally, these scripts should be merged.

set -o errexit
set -o pipefail
set -o noclobber
# Used when symlinking files from the working tree: symlink .* files
# too.
shopt -s dotglob

# Some versions of git set $GIT_WORK_TREE when ran through an alias.
# This wouldn't work with git-latexdiff which plays with different
# work trees.
unset GIT_DIR
unset GIT_WORK_TREE

# (Comment and 'unset' line borrowed from Git's source code)
# Having this variable in your environment would break scripts because
# you would cause "cd" to be taken to unexpected places.  If you
# like CDPATH, define it for your interactive shell sessions without
# exporting it.
# But we protect ourselves from such a user mistake nevertheless.
unset CDPATH

# @GIT_LATEXDIFF_VERSION@ is substituted by the install script here,
# but not within git_latexdiff_compute_version().
git_latexdiff_version='@GIT_LATEXDIFF_VERSION@'

git_latexdiff_compute_version () {
    if [ "$git_latexdiff_version" = '@GIT_LATEXDIFF''_VERSION@' ]; then
	(cd "$(dirname "$0")" && git describe --tags HEAD 2>/dev/null || echo 'Unknown version')
    else
	echo "$git_latexdiff_version"
    fi
}

usage () {
    cat << EOF
Usage: $(basename "$0" | sed 's/git-/git /') [options] OLD [NEW]
       $(basename "$0" | sed 's/git-/git /') [options] OLD --
       $(basename "$0" | sed 's/git-/git /') [options] -- OLD
Call latexdiff on two Git revisions of a file.

OLD and NEW are Git revision identifiers. NEW defaults to HEAD.
If "--" is used for NEW, then diff against the working directory.

Options:
    --help                this help message
    --help-examples       show examples of usage
    --main <file>         name of the main LaTeX, R Sweave,
                            or Emacs Org mode file.
                            The search for the only file containing 'documentclass'
                            will be attempted, if not specified.
                            For non-LaTeX files, a reasonable \`prepare\` command
                            will be used unless explicitly provided
    --no-view             don't display the resulting PDF file
    --latex               run latex instead of pdflatex
    --xelatex             run xelatex instead of pdflatex
    --lualatex            run lualatex instead of pdflatex
    --tectonic            run tectonic instead of pdflatex
    --bibtex, --bbl       display changes in the bibliography
                             (runs bibtex to generate *.bbl files and
                             include them in the source file using
                             latexpand --expand-bbl before computing
                             the diff)
    --biber               like --bibtex, but runs biber instead.
    --run-bibtex, -b      run bibtex as well as latex to generate the PDF file
                             (pdflatex,bibtex,pdflatex,pdflatex)
                          NOTE: --bibtex usually works better
    --run-biber           run BibLaTex-Biber as well as latex to generate the PDF file
                             (pdflatex,biber,pdflatex,pdflatex)
                          NOTE: --biber usually works better
    --view                view the resulting PDF file
                            (default if -o is not used)
    --pdf-viewer <cmd>    use <cmd> to view the PDF file (default: \$PDFVIEWER)
    --no-cleanup          don't cleanup temp dir after running
    --no-flatten          don't call latexpand to flatten the document
    --cleanup MODE        Cleanup temporary files according to MODE:

                           - keeppdf (default): keep only the
                                  generated PDF file

                           - none: keep all temporary files
                                  (may eat your diskspace)

                           - all: erase all generated files.
                                  Problematic with --view when the
                                  viewer is e.g. evince, and doesn't
                                  like when the file being viewed is
                                  deleted.

    --latexmk             use latexmk
    --build-dir           use pdfs from specific build directory
    --latexopt            pass additional options to latex (e.g. -shell-escape)
    -o <file>, --output <file>
                          copy resulting PDF into <file> (usually ending with .pdf)
                          Implies "--cleanup all"
    --tmpdirprefix        where temporary directory will be created (default: /tmp).
                            Relative path will use repository root as a base
    --verbose, -v         give more verbose output
    --quiet               redirect output from subprocesses to log files
    --prepare <cmd>       run <cmd> before latexdiff (e.g. run make to generate
                             included files)
    --filter <cmd>        run <cmd> after latexdiff and before compilation
                             (e.g. to fix up latexdiff output)
    --ln-untracked        symlink uncommited files from the working directory
    --version             show git-latexdiff version.
    --subtree             checkout the tree at and below the main file
                             (enabled by default, disable with --whole-tree)
    --whole-tree          checkout the whole tree (contrast with --subtree)
    --ignore-latex-errors keep on going even if latex gives errors, so long as
                          a PDF file is produced
    --ignore-makefile     ignore the Makefile, build as though it doesn't exist
    -*                    other options are passed directly to latexdiff
    --latexpand OPT       pass option OPT to latexpand. Use multiple times like
                          --latexpand OPT1 --latexpand OPT2 to pass multiple options.
    --latexdiff-flatten   use --flatten from latexdiff instead of latexpand

Unrecognized options are passed unmodified to latexdiff.
EOF
}

examples () {
    cat <<EOF
Examples:

Diff the previous revision with the latest commit:

    git latexdiff HEAD^

Diff the latest commit with the working tree:

    git latexdiff HEAD --

Diff latest commit with branch master:

    git latexdiff master HEAD

Pass --type=CHANGEBAR to latexdiff to get changebars in the margins
instead of red+trike/blue+underline diff:

    git latexdiff --type=CHANGEBAR HEAD^

Use a specific latexdiff configuration file:

    git latexdiff --config /path/to/file HEAD^
EOF
}

die () {
    echo "fatal: $*"
    exit 1
}

verbose () {
    if test "$verbose" = 1 ; then
	printf "%s ..." "$@"
    fi
}

verbose_progress () {
    if test "$verbose" = 1 ; then
	printf "."
    fi
}

verbose_done () {
    if test "$verbose" = 1 ; then
	echo " ${1:-done}."
    fi
}

verbose_say () {
    if test "$verbose" = 1 ; then
	printf "%s\n" "$@"
    fi
}

old=
new=
main=
view=maybe
cleanup=keeppdf
verbose=0
bibtex=0
biber=0
output=
initial_dir=$PWD
tmpdir_prefix="/tmp"
prepare_cmd=
flatten=1
subtree=1
uselatexmk=
use_build_dir=
latexopt=
ln_untracked=0
quiet=0
ignorelatexerrors=0
latexdiffopt=()
latexpand=()
bbl=0
latexdiff_flatten=0
latex=0
xelatex=0
lualatex=0
tectonic=0
BIBTEX_EXEC=bibtex

while test $# -ne 0; do
    case "$1" in
        "--help"|"-h")
            usage
            exit 0
            ;;
	"--help-examples")
	    examples
	    exit 0
	    ;;
	"--main")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    main=$1
	    ;;
	"--no-view")
	    view=0
	    ;;
	"--view")
	    view=1
	    ;;
	"--pdf-viewer")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    PDFVIEWER="$1"
	    ;;
	"--no-cleanup")
	    cleanup=none
	    ;;
	"--ignore-latex-errors")
	    ignorelatexerrors=1
	    ;;
        "--cleanup")
            shift
            case "$1" in
                "none"|"all"|"keeppdf")
                    cleanup="$1"
                    ;;
                *)
                    echo "Bad argument --cleanup $1"
                    usage
                    exit 1
                    ;;
            esac
            ;;
	"--no-flatten")
            flatten=0
            ;;
	"--ignore-makefile")
	    ignoremake=1
	    ;;
	"-o"|"--output")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    output=$1
	    cleanup=all
	    ;;
	"-b"|"--bibtex")
	    bbl=1
	    ;;
	"--latex")
	    latex=1
	    ;;
	"--xelatex")
            xelatex=1
            ;;
	"--lualatex")
	    lualatex=1
	    ;;
	"--tectonic")
	    tectonic=1
	    ;;
	"--biber")
	    BIBTEX_EXEC=biber
	    bbl=1
	    ;;
	"--run-bibtex")
	    bibtex=1
	    ;;
	"--run-biber")
	    biber=1
	    ;;	
	"--verbose"|"-v")
	    verbose=1
	    ;;
        "--quiet")
	    quiet=1
	    ;;
	"--version")
	    git_latexdiff_compute_version
            exit 0
	    ;;
	"--subtree")
	    subtree=1
	    ;;
	"--whole-tree")
	    subtree=0
	    ;;
	"--prepare")
	    shift
	    prepare_cmd="$1"
	    ;;
	"--filter")
	    shift
	    filter_cmd="$1"
	    ;;
        "--build-dir")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    use_build_dir=$1
            ;;
        "--latexmk")
            uselatexmk=1
            ;;
	"--latexpand")
	    shift
	    latexpand=("${latexpand[@]}" "$1")
	    ;;
	"--bbl")
	    bbl=1
	    ;;
	"--latexdiff-flatten")
	    latexdiff_flatten=1
            flatten=0
	    ;;
	"--latexopt")
	    shift
	    latexopt=$1
	    ;;
        "--ln-untracked")
            ln_untracked=1
            ;;
        "--no-ln-untracked")
            ln_untracked=0
            ;;
        "--tmpdirprefix")
	    shift
	    tmpdir_prefix="$1"
	    ;;
        -*)
            if test "$1" = "--" ; then
                if test -z "$new" ; then
                    new=$1
                else
                    echo "Bad argument $1"
                    usage
                    exit 1
                fi
            else
		case "$1" in
		    '--type'|'-t'|'--subtype'|'-s'|'--floattype'|'-f'|\
			'--config'|'-c'|'-p'|'--encoding'|'-e'|\
			'--label'|'-L'|'--exclude-safecmd'|'-A'|\
			'--replace-safecmd'|'--append-safecmd'|'-a'|\
			'--exclude-textcmd'|'-X'|'--replace-textcmd'|\
			'--append-textcmd'|'-x'|'--replace-context1cmd'|\
			'--append-context1cmd'|'--replace-context2cmd'|\
			'--append-context2cmd'|'--packages'|'--math-markup'|\
			'--driver')
			# Options taking an immediate argument in
			# latexdiff => add both the option and its
			# argument.
			latexdiffopt+=("$1" "$2")
			shift
			;;
		    '--preamble')
			# Same, but with a file argument. Make it
			# absolute to avoid issues when cd-ing
			# somewhere else.
			absolute="$(cd $(dirname "$2"); pwd)/$(basename "$2")"
			latexdiffopt+=("$1" "$absolute")
			shift
			;;
		    *)
			latexdiffopt+=("$1")
			;;
		esac
            fi
            ;;
        *)
	    if test -z "$1" ; then
		echo "Empty string not allowed as argument"
		usage
		exit 1
	    elif test -z "$old" ; then
		old=$1
	    elif test -z "$new" ; then
		new=$1
	    else
		echo "Bad argument $1"
		usage
		exit 1
	    fi
            ;;
    esac
    shift
done

initial_repo=$(git rev-parse --show-toplevel)

if test -z "$new" ; then
    new=HEAD
fi

if test -z "$old" ; then
    echo "fatal: Please, provide at least one revision to diff with."
    usage
    exit 1
fi

if test -z "$PDFVIEWER" ; then
    verbose "Auto-detecting PDF viewer"
    candidates="xdg-open evince okular xpdf acroread"
    if test "$(uname)" = Darwin ; then
        # open exists on GNU/Linux, but does not open PDFs
	candidates="open $candidates"
    fi

    for command in $candidates; do
	if command -v "$command" >/dev/null 2>&1; then
	    PDFVIEWER="$command"
	    break
	else
	    verbose_progress
	fi
    done
    verbose_done "$PDFVIEWER"
fi

case "$view" in
    maybe|1)
	if test -z "$PDFVIEWER" ; then
	    echo "warning: could not find a PDF viewer on your system."
	    echo "warning: Please set \$PDFVIEWER or use --pdf-viewer CMD."
	    PDFVIEWER=false
	fi
	;;
esac

if test $flatten = 1 &&
    ! command -v latexpand 2>/dev/null; then
    echo "Warning: latexpand not found. Falling back to latexdiff --flatten."
    latexdiff_flatten=1
    flatten=0
fi

if test $latex = 1; then
    LATEX_EXEC=latex
elif test $xelatex = 1; then
    LATEX_EXEC=xelatex
elif test $lualatex = 1; then
    LATEX_EXEC=lualatex
elif test $tectonic = 1; then
    LATEX_EXEC=tectonic
else
    LATEX_EXEC=pdflatex
fi

if test $biber = 1; then
    BIBTEX_EXEC=biber
fi

## end option parsing ##

check_knitr () {
    if test -z "$prepare_cmd"; then
	prepare_cmd="Rscript -e \"library(knitr); knit('$main')\""
    fi
    main="${main%\.*}.tex"
}

check_org () {
    if test -z "$prepare_cmd"; then
        prepare_cmd="emacs --batch --eval \"(load \\\"~/.emacs\\\")\" \"$main\" -f org-latex-export-to-latex --kill"
    fi
    main="${main%\.*}.tex"
}

log_cmd () {
    log=$1
    shift
    if [ "$quiet" = 1 ]; then
	"$@" >$log 2>&1
    else
	"$@"
    fi
}

# main is relative to initial_dir (if returned)
if test -z "$main" ; then
    printf "%s" "No --main provided, trying to guess ... "
    main=$(git grep -l '^[ \t]*\\documentclass')
    # May return multiple results, but if so the result won't be a file.
    if test -r "$main" ; then
	echo "Using $main as the main file."
    else
	if test -z "$main" ; then
	    echo "No candidate for main file."
	else
	    echo "Multiple candidates for main file:"
	    printf "%s\n" "$main" | sed 's/^/\t/'
	fi
	die "Please, provide a main file with --main FILE.tex."
    fi
fi

if test ! -r "$main" ; then
    die "Cannot read $main."
fi

ext=${main##*\.}
case "$ext" in
    Rnw) check_knitr ;;
    Rtex) check_knitr ;;
    org) check_org ;;
    *) ;;
esac

# Set LATEXDIFF_EXEC to either latexdiff or latexdiff-so. Prefer
# latexdiff-so if available.
if command -v latexdiff-so >/dev/null 2>&1; then
    LATEXDIFF_EXEC=latexdiff-so
elif command -v latexdiff >/dev/null 2>&1; then
    LATEXDIFF_EXEC=latexdiff
else
    die "latexdiff-so and latexdiff couldn't be found. Check your PATH."
fi
verbose_done "$LATEXDIFF_EXEC"

verbose "Creating temporary directories"

git_prefix=$(git rev-parse --show-prefix)
git_dir="$(git rev-parse --git-dir)" || die "Not a git repository?"
cd "$(git rev-parse --show-cdup)" || die "Can't cd back to repository root"
git_dir=$(cd "$git_dir"; pwd)
git_worktree=$(pwd)

relative_main_dir=$(dirname "$main")
# make main relative to git root directory
if test -n "$git_prefix" ; then
    main=$git_prefix$main
fi
mainbase=$(basename "$main" .tex)
maindir=$(dirname "$main")

tmpdir=$tmpdir_prefix/git-latexdiff.$$
mkdir "$tmpdir" || die "Cannot create temporary directory."

cd "$tmpdir" || die "Cannot cd to $tmpdir"
if test "$(uname -o 2>/dev/null)" = "Msys"; then
    tmpdir=$(pwd -W)
else
    tmpdir=$(pwd)
fi

mkdir old new || die "Cannot create old and new directories."

verbose_done
verbose_say "Temporary directories: $tmpdir/old and $tmpdir/new"
verbose "Checking out old and new version"

cd old || die "Cannot cd to old/"
if test "$ln_untracked" = 1; then
    (
	mkdir -p "$maindir" && cd "$maindir" &&
	    log_cmd ln-old.log ln -s "$initial_repo"/"$maindir"/* .
    ) || true
fi

if test "$subtree" = 1 && test -n "$git_prefix"; then
    checkoutroot=$git_prefix
else
    checkoutroot="."
fi
# create the build directory (containing the final PDFs) if the param was set
if test -n "$use_build_dir" ; then
    builddir="$use_build_dir"
else
    builddir="$relative_main_dir"
fi

# Checkout a subtree, without touching the index ("git checkout" would)
(cd "$git_dir" && git archive --format=tar "$old" "$checkoutroot") | tar -xf -
# Also expand the possible submodules
(cd "$git_worktree" && git submodule foreach --recursive 'git archive --format=tar "$sha1" | tar -xf - --directory '$tmpdir/old'/$displaypath')
verbose_progress
cd ../new || die "Cannot cd to new/"
if test "$new" == "--"; then
    # Copy working tree files
    (cd "$git_worktree" && git ls-files -- "$checkoutroot" | tar -cf - -T -) | tar -xf -
else
    # checkout new revision
    (cd "$git_dir" && git archive --format=tar "$new" "$checkoutroot") | tar -xf -
    (cd "$git_worktree" && git submodule foreach --recursive 'git archive --format=tar "$sha1" | tar -xf - --directory '$tmpdir/new'/$displaypath')
fi
if test "$ln_untracked" = 1; then
    (
	mkdir -p "$maindir" && cd "$maindir" &&
	    log_cmd ln-new.log ln -s "$initial_repo"/"$maindir"/* .
    ) || true
fi

verbose_progress
cd ..

verbose_done

for dir in old new
do
    verbose "Running preparation command $prepare_cmd in $dir/$git_prefix"
    ( cd "$dir/$git_prefix/" && log_cmd prepare.log eval "$prepare_cmd" )
    if test ! -f "$dir/$main"; then
	die "$prepare_cmd did not produce $dir/$main."
    fi
    verbose_done
done

if test $tectonic != 1; then
  if [ "$ignorelatexerrors" = 1 ]; then
      latexopt="$latexopt -interaction=batchmode"
  elif [ "$quiet" = 1 ]; then
      latexopt="$latexopt -interaction=nonstopmode"
  else
      latexopt="$latexopt -interaction=errorstopmode"
  fi
fi

# Option to use latexdiff --flatten instead of latexpand
if test "$latexdiff_flatten" = 1; then
    latexdiffopt+=("--flatten")
fi

# Shortcut to include bbl
if test "$bbl" = 1; then
    if test "$biber" = 1; then
	bblexpand=("--expand-bbl" "$mainbase.bbl")
	# In theory, this (with recent enough latexpand) should work
	# better. In practice it doesn't seem to work though.
	# bblexpand=("--biber" "$mainbase.bbl")
    else
	bblexpand=("--expand-bbl" "$mainbase.bbl")
    fi
else
    bblexpand=()
fi

ignore_errors_maybe() {
    if [ "$compile_error" = 1 ] && [ "$ignorelatexerrors" = 1 ]; then
	echo "LaTeX errors were found - but attempting to carry on."
	compile_error=0
    fi
}

# Create flattened documents and keep for debugging
if test "$flatten" = 1; then
    if [ "$bbl" = 1 ]; then
	if [ ! -f "old/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing old/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd old/"$maindir"
	    log_cmd pdflatex0.log $LATEX_EXEC $latexopt "$mainbase" || {
		compile_error=1
		error_msg="command 'pdflatex' (automatically run in old due to --bbl) failed."
	    }
	    log_cmd "$BIBTEX_EXEC"0.log $BIBTEX_EXEC "$mainbase" || {
		compile_error=1
		error_msg="command '$BIBTEX_EXEC' (automatically run in old due to --bbl) failed."
	    }
	    cd "$oldPWD"
	    ignore_errors_maybe
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for old version"
	    fi
	fi
	if [ ! -f "new/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing new/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd new/"$maindir"
	    log_cmd pdflatex0.log $LATEX_EXEC $latexopt "$mainbase" || {
		compile_error=1
		error_msg="command 'pdflatex' (automatically run in new due to --bbl) failed."
	    }
	    log_cmd "$BIBTEX_EXEC"0.log $BIBTEX_EXEC "$mainbase" || {
		compile_error=1
		error_msg="command '$BIBTEX_EXEC' (automatically run in new due to --bbl) failed."
	    }
	    cd "$oldPWD"
	    ignore_errors_maybe
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for new version"
	    fi
	fi
    fi
    verbose "Running latexpand"
    (
	cd old/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > old-"$mainbase"-fl.tex \
	|| die "latexpand failed for old version"
    (
	cd new/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > new-"$mainbase"-fl.tex \
	|| die "latexpand failed for new version"
    verbose_done

    verbose "Running $LATEXDIFF_EXEC ${latexdiffopt[*]} old-${mainbase}-fl.tex new-${mainbase}-fl.tex > ./diff.tex"
    "$LATEXDIFF_EXEC" "${latexdiffopt[@]}" old-"$mainbase"-fl.tex new-"$mainbase"-fl.tex > diff.tex \
	|| die "$LATEXDIFF_EXEC failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new/"$main" new/"$main".orig
    mv -f diff.tex new/"$main"
    verbose_done
else
    verbose "Running $LATEXDIFF_EXEC ${latexdiffopt[*]} old/$main new/$main > ./diff.tex"
    "$LATEXDIFF_EXEC" "${latexdiffopt[@]}" old/"$main" new/"$main" > diff.tex \
	|| die "$LATEXDIFF_EXEC failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new/"$main" new/"$main.orig"
    mv -f diff.tex new/"$main"
    verbose_done
fi

if [ ! -z "$filter_cmd" ]; then
    verbose "Running filter command $filter_cmd in new/"
    ( cd "new/" && log_cmd filter.log eval "$filter_cmd" )
    if [ ! -f "new/$main" ]; then
	die "$filter_cmd removed new/$main."
    fi
    verbose_done
fi

verbose "Compiling result"

compile_error=0

oldPWD=$PWD
cd new/"$maindir" || die "Can't cd to new/$maindir"
if test -f Makefile && test "$ignoremake" != 1 ; then
    log_cmd make.log make || {
	compile_error=1
	error_msg="command 'make' failed."
    }
elif test "$uselatexmk" = 1; then
    log_cmd latexmk.log latexmk -f -pdf -silent $latexopt "$mainbase" || {
	compile_error=1
	error_msg="command 'latexmk' failed."
    }
elif test "$tectonic" = 1; then
    log_cmd tectonic.log tectonic $latexopt "$mainbase.tex" || {
	compile_error=1
	error_msg="command 'tectonic' failed."
    }
else
    log_cmd pdflatex1.log $LATEX_EXEC $latexopt "$mainbase" || {
	compile_error=1
	error_msg="command pdflatex (first run) failed."
    }
    if test "$bibtex" = 1 || test "$biber" = 1 ; then
	log_cmd "$BIBTEX_EXEC".log $BIBTEX_EXEC "$mainbase" || {
	    compile_error=1
	    error_msg="command '$BIBTEX_EXEC' failed."
	}
    fi
    log_cmd pdflatex2.log $LATEX_EXEC $latexopt "$mainbase" || {
	compile_error=1
	error_msg="command 'pdflatex' (second run) failed."
    }
    log_cmd pdflatex3.log $LATEX_EXEC $latexopt "$mainbase" || {
	compile_error=1
	error_msg="command 'pdflatex' (third run) failed."
    }
fi
cd "$oldPWD"

# Same relative path as where we've been called from, but in the
# temporary new/ directory:
cd new/"$git_prefix"

verbose_done

ignore_errors_maybe

if test $latex = 1; then
    dvips "$mainbase".dvi
    ps2pdf "$mainbase".ps
fi

pdffile="$builddir/$mainbase".pdf
if test ! -r "$pdffile" ; then
    echo "No PDF file generated."
    echo "Working directory: $PWD"
    echo "Expected PDF: $pdffile"
    compile_error=1
elif test ! -s "$pdffile" ; then
    echo "PDF file generated is empty."
    compile_error=1
fi

if test "$compile_error" = "1" ; then
    echo "Error during compilation. Please examine and cleanup if needed:"
    echo "Directory: $tmpdir/new/$maindir"
    echo "     File: $mainbase.tex"
    echo "  Problem: $error_msg"
    # Don't clean up to let the user diagnose.
    exit 1
fi

if test -n "$output" ; then
    abs_pdffile="$PWD/$pdffile"
    (cd "$initial_dir" && mv "$abs_pdffile" "$output")
    pdffile="$output"
    echo "Output written on $pdffile"
elif [ -f "$pdffile" ]; then
    new_pdffile="$tmpdir"/"$mainbase".pdf
    mv "$pdffile" "$new_pdffile"
    pdffile="$new_pdffile"
fi

# Change directory so nothing will keep us from cleaning
cd "$initial_dir"

if test "$view" = 1 || ( test "$view" = maybe  && test -z "$output" ) ; then
    "$PDFVIEWER" "$pdffile"
fi

case "$cleanup" in
    "all")
	verbose "Cleaning-up result"
	rm -fr "$tmpdir"
	verbose_done
	;;
    "keeppdf")
	verbose "Cleaning-up all but pdf (kept in $pdffile)"
	rm -fr "$tmpdir"/old "$tmpdir"/new
	verbose_done
	;;
    "none")
	verbose_say "Generated files kept in $tmpdir/"
	;;
esac


==> review/report/Makefile <==
# Makefile for compiling a *.tex file into a *.pdf file
# The current folder must contain only one *.tex file
#
# Author: Joao Moura
# Email: jmm7@hw.ac.uk
# Last Modified at 01/06/2016
#
#################################################################
#################################################################
# Identify what is the name of the *.tex file to compile
# NOTE: There must be a single *.tex file in the current directory
TEX = pdflatex -shell-escape
TIKZ = Tikz
FILE_TEX=$(wildcard *.tex)
TARGET=$(FILE_TEX:.tex=)
#################################################################

#################################################################
# Rule that runs whether the make is called or the target file is outdated.
FORCE: $(FILE_TEX)
	$(TEX) $(TARGET)
	$(TEX) $(TARGET)
#################################################################

#################################################################
# Rule to create a bibtex file
.PHONY: bib
bib:
	$(BIB) $(TARGET)
#################################################################

#################################################################
# Rule for cleaning: It removes all the files with TARGET name except the file with *.tex extension
.PHONY: clean
clean: 
	rm -f $(filter-out $(TARGET).tex, $(wildcard $(TARGET).*))
#################################################################

#################################################################
# Rule for cleaning all tikz files
.PHONY: cleanall
cleanall: 
	rm -f $(filter-out $(wildcard Tikz/*.tex) $(TARGET).tex, $(wildcard Tikz/*.*) $(wildcard $(TARGET).*))
#################################################################

#################################################################
# Rule for cleaning the bib file
.PHONY: cleanbib
cleanbib:
	# Remove unnecessary keywords:
	gsed -i '/^abstract/d' $(FILE_BIB)
	gsed -i '/^archivePrefix/d' $(FILE_BIB)
	gsed -i '/^arxivId/d' $(FILE_BIB)
	gsed -i '/^eprint/d' $(FILE_BIB)
	gsed -i '/^isbn/d' $(FILE_BIB)
	gsed -i '/^issn/d' $(FILE_BIB)
	gsed -i '/^mendeley-tags/d' $(FILE_BIB)
	gsed -i '/^pmid/d' $(FILE_BIB)
	gsed -i '/^primaryClass/d' $(FILE_BIB)
	gsed -i '/^keywords/d' $(FILE_BIB)
	gsed -i '/^url/d' $(FILE_BIB)
	gsed -i '/^file/d' $(FILE_BIB)
	# Insert tab before keyword:
	gsed -i 's/^\([a-z]\)/\t\1/' $(FILE_BIB)
	# Remove double brackets in titles:
	gsed -i 's/{{\(.*\)}}/{\1}/' $(FILE_BIB)
	# Add a line after each reference:
	gsed -i '/^}/a\\' $(FILE_BIB)
#################################################################

